Abelian 3d mirror symmetry on $\mathbb{RP}^2 \times \mathbb{S}^1$ with $N_f=1$

We consider a new 3d superconformal index defined as the path integral over $\mathbb{RP}^2 \times \mathbb{S}^1$, and get the generic formula for this index with arbitrary number of U$(1)$ gauge symmetries via the localization technique. We find two consistent parity conditions for the vector multiplet, and name them $\mathcal{P}$ and $\mathcal{CP}$. We find an interesting phenomenon that two matter multiplets coupled to the $\mathcal{CP}$-type vector multiplet merge together. By using this effect, we investigate the simplest version of 3d mirror symmetry on $\mathbb{RP}^2 \times \mathbb{S}^1$ and observe four types of coincidence between the SQED and the XYZ model. We find that merging two matters plays an important role for the agreement.

==> sections/33333v2.tex <==
%!TEX encoding = JISJapanese
\include{common_supp_files/begin}
\include{common_supp_files/sonota/begin2}



%%%%%%%%%%%% Section 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Mirror symmetry on $\mathbb{RP}^{2} \times \mathbb{S}^{1}$}\label{Mirrorsym}
\begin{table}[t]
\vspace{-1em}
\begin{center}
\begin{tabular}{c}
%\vspace{-.5em}
	\begin{minipage}[b]{.48\hsize} %Charges in the SQED
		\begin{center}
			\begin{tabular}{|c|c|c|c|c|} \hline
			& U$(1)$ & U$(1)_{J}$ & U$(1)_{A}$ & $\hat{R}$ \\ \hline \hline
			$Q$ & $+ 1$ & $0$ & $+ 1$ & $- \Delta$ \\ \hline
			$\tilde{Q}$ & $- 1$ & $0$ & $+ 1$ & $- \Delta$ \\ \hline
			\end{tabular}
		\end{center}
	\vspace{-.75em}
	\caption{Charges in the SQED. Global symmetries are a topological U$(1)_{J}$ and an axial U$(1)_{A}$.\label{cSQED}}
	\end{minipage}
	\hspace{2em}
	\begin{minipage}[b]{.52\hsize} %Charges in XYZ model
		\begin{center}
			\begin{tabular}{|c|c|c|c|} \hline
			& U$(1)_{V}$ & U$(1)_{A}$ &$\hat{R}$ \\ \hline \hline
			$X$ & $+ 1$ & $+ 1$ & $- ( 1 - \Delta )$ \\ \hline
			$Y$ & $- 1$ & $+ 1$ & $- ( 1 - \Delta )$ \\ \hline
			$Z$ & 0 & $- 2$ & $- 2 \Delta$ \\ \hline
			\end{tabular}
		\end{center}
	\vspace{-.75em}
	\caption{Charges in the XYZ model. Global symmetries are a vector-like U$(1)_{V}$ and an axial U$(1)_{A}$.\label{cXYZ}}
	\end{minipage}
\end{tabular}
\end{center}
\end{table}

\begin{table}[t] %Mirror map
\vspace{-.7em}
\begin{center}
	\begin{tabular}{ccc} \hline
	SQED & & XYZ \\ \hline
	U$(1)_{J}$, $J_{J}$ & $\leftrightarrow$ & U$(1)_{V}$, $J_{V}$ \\
	U$(1)_{A}$, $J_{A}$ & $\leftrightarrow$ & U$(1)_{A}$, $- J_{A}$ \\
	$e^{\left( \sigma + i \rho \right) / e^{2}}$, $e^{- \left( \sigma + i \rho \right) / e^{2}}$ & $\leftrightarrow$ & $X$, $Y$ \\
	$Q \tilde{Q}$ & $\leftrightarrow$ & $Z$ \\ \hline
	\end{tabular}
\end{center}
\vspace{-1em}
\caption{The mirror map. $J_{J}$, $J_{V}$, and $J_{A}$ are currents associated to U$(1)_{J}$, U$(1)_{V}$, and U$(1)_{A}$, respectively. $e^{2}$ is a coupling constant.\label{mmap}}
\end{table}

Mirror symmetry is a kind of dualities between theories which flow to the same IR fixed point along the RG flow. In this paper, we deal with $\mathcal{N} = 2$ mirror symmetry \cite{Intriligator:1996ex, Aharony:1997bx} between the SQED and the XYZ model on $\mathbb{RP}^{2} \times \mathbb{S}^{1}$; the former has a vector multiplet and two chiral fields $Q$ and $\tilde{Q}$ charged under the U$(1)$ gauge group, and the latter is comprised of three chiral fields $X, Y$, and $Z$ coupled to each other through the superpotential $\mathcal{W} = XYZ$. In addition, they contain two global U$(1)$ symmetries and $R$-symmetry acting on the chiral fields. We arrange all charge assignments in Table \ref{cSQED} and \ref{cXYZ}.

In the context of mirror symmetry, the languages of the SQED are mapped to those of the XYZ model as in Table \ref{mmap}. The bottom two lines in Table \ref{mmap} are the correspondences of moduli parameters. $\pm ( \sigma + i \rho )$, where $\rho$ is the dual photon defined by
\begin{align} %def of dual photon
\frac{1}{2} \epsilon_{\mu \nu \rho} F^{\nu \rho} = \partial_{\mu} \rho,
\label{dualphoton}
\end{align}
characterize the Coulomb branch, and the Higgs branch is parametrized by $Q \tilde{Q}$. Notice that we assume the maps of the moduli are kept not only at the classical level but also for quantum fluctuations of these fields. We shall follow this assumption to decide the parity condition for the XYZ model.

We consider the case where global symmetries are gauged. %(the index with gauged background fields is called the generalized index \cite{Kapustin:2011jm}).
The fact that the background gauge field of a topological U$(1)_{J}$ in the SQED is coupled to a topological current $J_{T} = \ast F$ shows the appearance of a BF term as a classical contribution. In fact, our BF term \eqref{BFvalue} carries out a significant effect to manifest mirror symmetry. With the gauging prescriptions as explained above, we find four types of mirror symmetry depending on the choices of consistent parity conditions in the SQED and the XYZ model. The first one explained in the subsection \ref{Ptype} is an one-parameter extension of mirror symmetry demonstrated in \cite{Tanaka:2014oda}, and others are completely new. We give the readers proof for all types of $\mathcal{N} = 2$ mirror symmetry in Apeendix \ref{24mirrorsym}.



%\clearpage
%%%%%%%%%%%% Section 3.1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The map of parity conditions}
\vspace{-.5em}
\begin{table}[h] %Parity actions in the SQED^P and the XYZ model
\begin{tabular}{c}
	\hspace{2em}
	\begin{minipage}[t]{.5\hsize} %SQED^P
		\begin{align*}
			\xymatrix {
                         *+[F-]{\text{$Q$}} 
                         \ar@{->}[r]
                         &
                         *++[o][F-]{\text{\scriptsize$\mc{P}$}} 
                         \ar@{->}[r]
                         &
                         *+[F-]{\text{$\tilde{Q}$}} }
		\end{align*}
		\vspace{-.3em}
		\begin{center}
			\begin{tabular}{rcl} \hline
			\multicolumn{3}{c}{SQED$^{( \mathcal{P} )}$} \\ \cline{1-3}
			$\sigma, \rho$ & $\begin{xy} {(0,5) \ar (7.5,5)} \end{xy}$ & $- \sigma, - \rho$  \\
			$Q$ & $\begin{xy} {(0,5) \ar (7.5,5)} \end{xy}$ & $Q$ \\
			$\tilde{Q}$ & $\begin{xy} {(0,5) \ar (7.5,5)} \end{xy}$ & $\tilde{Q}$ \\ \hline
			\end{tabular}
		\end{center}
	\end{minipage}
	\hspace{-3.5em}
	$\begin{xy} {(0,-10) \ar@{<=>} (10,-10)} \end{xy}$
	\hspace{-5em}
	\begin{minipage}[t]{.5\hsize} %XYZ
		\begin{align*}
			\hspace{-3em}
			\xymatrix {
                 	&
                 	*+[F-]{\text{\scriptsize$
                 	\begin{matrix}
                 	X &
                 	Y
                 	\end{matrix}
                 	$}} 
                 	%\ar@{-}[r]^{\mc{W}}
                 	&
                 	*+[F-]{\text{$Z$}} }
		\end{align*}
		\vspace{-.3em}
		\begin{center}
			\begin{tabular}{rcl} \hline
			\multicolumn{3}{c}{$^{\text{X}}_{\text{Y}} \text{Z}$} \\ \cline{1-3}
			\shortstack{\strut $X$ \\ $Y$ } & $\begin{xy} {(0,10) \ar (7.5,5)}, {(0,5) \ar (7.5,10)} \end{xy}$ & \shortstack{\strut $Y$ \\ $X$ } \\
			$Z$ & $\begin{xy} {(0,5) \ar (7.5,5)} \end{xy}$ & $Z$ \\ \hline
			\end{tabular}
		\end{center}
	\end{minipage}
\end{tabular}
\caption{Parity conditions in SQED$^{( \mathcal{P} )}$ and $^{\text{X}}_{\text{Y}} \text{Z}$.\label{b1-type}}
\end{table}

In this subsection, we summarize the parity actions in the SQED and the corresponding conditions in the XYZ model based on the mirror map of the moduli parameters.

Firstly, we focus on the SQED under the parity conditions \eqref{vecp1} and \eqref{ematp1} denoted by SEQD$^{( \mathcal{P} )}$. In the language of the moduli parameters, $\sigma$ and $\rho$ receive flipping its sign under $\mathcal{P}$, but $Q$ and $\tilde{Q}$ do not mix up. Recalling the mirror map (Table \ref{mmap}), we can see that changing the signs of $\sigma$ and $\rho$ corresponds to the interchange of $X$ and $Y$, and $Z$ does not take any effect (the right side of Table \ref{b1-type}). This means that $( X, Y )$ behave as a doublet matter multiplet described by the parity condition \eqref{ematp2}. We name this dual theory $^{\text{X}}_{\text{Y}} \text{Z}$ to represent combining $( X, Y )$ as a single multiplet on $\mathbb{S}^{2} \times \mathbb{S}^{1}$. We argue mirror symmetry between SEQD$^{( \mathcal{P} )}$ and $^{\text{X}}_{\text{Y}} \text{Z}$ with respect to the parity conditions in Table \ref{b1-type}.



\begin{table}[h] %Charge conjugations in the SQED^CP and the XYZ model
\begin{tabular}{c}
	\hspace{2em}
	\begin{minipage}[t]{.5\hsize} %SQED^CP
		\begin{align*}
		\xymatrix {
			*+[F-]{\text{\scriptsize$
			\begin{matrix}
			Q \\
			\tilde{Q}
			\end{matrix}
			$}}
			&
			*++[o][F-]{\text{\scriptsize$\mc{CP}$}} 
			\ar@{->}[l]<1.5mm>
			\ar@{<-}[l]<-1.5mm> }
		\end{align*}
		\vspace{-.3em}
		\begin{center}
			\begin{tabular}{rcl} \hline
			\multicolumn{3}{c}{SQED$^{( \mathcal{CP} )}$} \\ \cline{1-3}
			$\sigma, \rho$ & $\begin{xy} {(0,5) \ar (7.5,5)} \end{xy}$ & $+ \sigma, + \rho$  \\
			\shortstack{ $Q$ \\ $\tilde{Q}$ } & $\begin{xy} {(0,10) \ar (7.5,5)}, {(0,5) \ar (7.5,10)} \end{xy}$ & \shortstack{\strut $\tilde{Q}$ \\ $Q$ } \\ \hline
			\end{tabular}
		\end{center}
	\end{minipage}
	\hspace{-4em}
	$\begin{xy} {(0,-10) \ar@{<=>} (10,-10)} \end{xy}$
	\hspace{-4.5em}
	\begin{minipage}[t]{.5\hsize} %XYZ
		\begin{align*}
			\xymatrix {
			*+[F-]{\text{$X$}} 
			%\ar@{-}[r]^{\mc{W}}]
			&
			*+[F-]{\text{$Y$}} 
			%\ar@{-}[r]^{\mc{W}}
			&
			*+[F-]{\text{$Z$}} }
		\end{align*}
		\vspace{-.15em}
		\begin{center}
			\begin{tabular}{ccc} \hline
			\multicolumn{3}{c}{XYZ} \\ \cline{1-3}
			$X$ & $\begin{xy} {(0,5) \ar (7.5,5)} \end{xy}$ & $X$ \\
			$Y$ & $\begin{xy} {(0,5) \ar (7.5,5)} \end{xy}$ & $Y$ \\
			$Z$ & $\begin{xy} {(0,5) \ar (7.5,5)} \end{xy}$ & $Z$ \\ \hline
			\end{tabular}
		\end{center}
	\end{minipage}
\end{tabular}
\caption{Parity conditions in SQED$^{( \mathcal{CP} )}$ and XYZ.\label{b3-type}}
\end{table}
Next, we consider the SQED satisfying our new parity conditions \eqref{vecp2} and \eqref{ematp2} which we call SQED$^{( \mathcal{CP} )}$. The moduli $\sigma$ and $\rho$ transform trivially, while the matters $Q$ and $\tilde{Q}$ must be exchanged each other because of accompanying charge conjugation $\mathcal{C}$ with $\mathcal{P}$ (the left side of Table \ref{b3-type}). The mirror map of the moduli spaces (Table \ref{mmap}) gives us the parity conditions in the XYZ model (denoted just by XYZ) such that $X$ and $Y$ remain intact, and also $Z$ is not affected since it is the product of $Q$ and $\tilde{Q}$. This correspondence of the parity conditions is indicated in Table \ref{b3-type} of which we make use in verifying mirror symmetry between SQED$^{( \mathcal{CP} )}$ and XYZ.



%\clearpage
%%%%%%%%%%%% Section 3.2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{$\text{SQED}^{( \mathcal{P} )}$ vs $^{\text{X}}_{\text{Y}} \text{Z}$}\label{Ptype}
\begin{align}
%%%% SQED^P+
\xymatrix {
&
*++[o][F.]{\text{\scriptsize$B_{A}^{+}, \theta_A$}} 
&
\\
*+[F-]{\text{$Q$}} 
\ar@{->}[r]
\ar@{.>}[ur]
&
*++[o][F-]{\text{\scriptsize$\mc{P}$}} 
\ar@{->}[r]
\ar@{.}[d]^{\text{BF}}
&
*+[F-]{\text{$\tilde{Q}$}}
\ar@{.>}[ul]
\\
&
*++[o][F.]{\text{\scriptsize$B_J, \theta_{J +}$}} 
&
\\
&
\text{SQED}^{(\mc{P}+)}
&
}	
\ \ \ \quad
\begin{xy}
{(5,-15) \ar @{<=>} (15,-15)}
\end{xy}
\hspace{-1.5em}
%%%% XYZ
\xymatrix {
&
*++[o][F.]{\text{\scriptsize$\tilde{B}_{A}^{+}, \tilde{\theta}_A$}} 
\ar@{<.}[d]<1.5mm>
\ar@{<.}[d]<-1.5mm>[r]
&
\\
&
*+[F-]{\text{\scriptsize$
\begin{matrix}
X &
Y
\end{matrix}
$}} 
\ar@{<.}[d]<1.5mm>
\ar@{.>}[d]<-1.5mm>
%\ar@{-}[r]^{\mc{W}}
&
*+[F-]{\text{$Z$}}
\ar@{<<.}[ul]
\\
&
*++[o][F.]{\text{\scriptsize$B_V, \theta_{V +}$}} 
&
}
\notag \\[-1.95em]
&\hspace{-4.5em}
{^\text{X}
_\text{Y}}^{(+)}
\text{Z}
\label{quiverP+} \\[-1em]
\notag
\end{align}

\paragraph{SQED$^{( \mathcal{P} + )}$ vs $^{\text{X}}_{\text{Y}}{}^{( + )}\text{Z}$}
This is the case studied in \cite{Tanaka:2014oda} 
%%%%%%
without the BF term in the SQED. Here, we incorporate the BF term into the index by turning on the $\mc{CP}$-type background gauge field \eqref{CPBG} for U$(1)_J$ global symmetry parametrized by $(B_J, \theta_{J+})$.
$\mc{CP}$-type is necessary to make the BF term parity-even. 
In addition, we turn on the $\mc{P}$-type background gauge field \eqref{PBG} for U$(1)_A$ global symmetry parametrized by $(B_A^+,\theta_A)$.
$\mc{P}$-type is necessary to make the gauge coupling parity-even. 
On the left side of \eqref{quiverP+}, we draw the quiver diagram.
We call it SQED$^{(\mc{P}+)}$ where the superscript indicates the existence of $\theta_{J+}$. 
The index is given by using the quiver rules summarized in subsection \ref{Recipe} as follows.
\begin{align} %SCI for SQED
&
\mathcal{I}_{\text{SQED}^{( \mathcal{P} + )}} ( x, \alpha, B_{J} ) \notag \\ %1
&=
q^{\frac{1}{8}}
\frac{( q^{2} ; q^{2} )_{\infty}}{( q ; q^{2} )_{\infty}}
\oint_{C_0} \frac{d z}{2 \pi i z} z^{s}
\left\{
a^{- \frac{1}{4}}
\frac
{( z^{- 1} a^{\frac{1}{2}} q^{\frac{1}{2}}, z a^{\frac{1}{2}} q^{\frac{1}{2}}; q^{2} )_{\infty}}
{( z a^{- \frac{1}{2}} q^{\frac{1}{2}}, z^{- 1} a^{- \frac{1}{2}} q^{\frac{1}{2}} ; q^{2} )_{\infty}}
+
a^{\frac{1}{4}}
\frac
{( z^{- 1} a^{\frac{1}{2}} q^{\frac{3}{2}}, z a^{\frac{1}{2}} q^{\frac{3}{2}} ; q^{2} )_{\infty}}
{( z a^{- \frac{1}{2}} q^{\frac{3}{2}}, z^{- 1} a^{- \frac{1}{2}} q^{\frac{3}{2}} ; q^{2} )_{\infty}} \right\}, %2
\label{scib1sqed1}
\end{align}
where the integration contour $C_{0}$ is the unit circle, $z := e^{i \theta}$, and $s := B_{J}/2 \in \mathbb{Z}$ is a backgorund monopole flux. $\alpha = e^{i \theta_{A}}$ represents a fugacity associated to U$(1)_{A}$, and also we define $q = x^{2}$ and $a = \alpha^{- 2} x^{2 ( 1 - \Delta )}$ for latter use.

On the other hand, we write down the quiver diagram of the dual theory ${^{\text{X}}_{\text{Y}}}^{(+)}\text{Z}$ in \eqref{quiverP+} where again 
the superscript means the existence of $\theta_{V+}$.
We also turn on $B_V$ and $(\tilde{B}_A^{+},\tilde{\theta}_A)$.
Then, the quiver rules give the corresponding index as
%%%%%
\begin{align} %SCI for XYZ
\mathcal{I}_{{^{\text{X}}_{\text{Y}}}^{(+)}\text{Z}} ( x, \tilde{\alpha}, B_{V} )
=
q^{\frac{1}{8}} \tilde{a}^{- \frac{1}{4}}
\left( \tilde{a}^{- \frac{1}{2}} q^{\frac{1}{2}} \right)^{| \tilde{s} |}
\frac{( \tilde{a}^{- \frac{1}{2}} q^{1 + |\tilde{s}|} ; q )_{\infty}}{( \tilde{a}^{\frac{1}{2}} q^{|\tilde{s}|} ; q )_{\infty}}
\frac{( \tilde{a} ; q^{2} )_{\infty}}{( \tilde{a}^{- 1} q ; q^{2} )_{\infty}},
\label{scib1xyz1}
\end{align}
where we define $\tilde{\alpha} = e^{i \tilde{\theta}_A}$, $\tilde{a} = \tilde{\alpha}^{2} x^{2 ( 1 - \Delta )}$ and $\tilde{s} = B_{V}/2 \in \mathbb{Z}$.

%%%%%%%
According to $\mc{N}=2$ mirror symmetry, 
the following identity is expected to hold:
%%%%%%%
\begin{align}
\mathcal{I}_{\text{SQED}^{( \mathcal{P} + )}} ( x, \alpha, B_{J} )
=
\mathcal{I}_{{^{\text{X}}_{\text{Y}}}^{(+)}\text{Z}} ( x, \tilde{\alpha}, B_{V} ),
\label{mirror1}
\end{align}
under identifications $\alpha = \tilde{\alpha}^{- 1}$ and $B_{J} = B_{V}$ found from the mirror map (Table \ref{mmap}). Note that, for all cases in the paper, we fix the background gauge field for U$(1)_{A}$ to be $B_{A}^{+}$. 



\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
%%%% SQED^P-
\xymatrix {
&
*++[o][F.]{\text{\scriptsize$B_{A}^{+}, \theta_A$}} 
&
\\
*+[F-]{\text{$Q$}} 
\ar@{->}[r]
\ar@{.>}[ur]
&
*++[o][F-]{\text{\scriptsize$\mc{P}$}} 
\ar@{->}[r]
\ar@{.}[d]^{\text{BF}}
&
*+[F-]{\text{$\tilde{Q}$}}
\ar@{.>}[ul]
\\
&
*++[o][F.]{\text{\scriptsize$B_J, \theta_{J -}$}} 
&
\\
&
\text{SQED}^{(\mc{P}-)}
&
}
\ \ \ \quad
\begin{xy}
{(5,-15) \ar @{<=>} (15,-15)}
\end{xy}
\hspace{-1.5em}
%%%% XYZ
\xymatrix {
&
*++[o][F.]{\text{\scriptsize$\tilde{B}_{A}^{+}, \tilde{\theta}_A$}} 
\ar@{<.}[d]<1.5mm>
\ar@{<.}[d]<-1.5mm>[r]
&
\\
&
*+[F-]{\text{\scriptsize$
\begin{matrix}
X &
Y
\end{matrix}
$}} 
\ar@{<.}[d]<1.5mm>
\ar@{.>}[d]<-1.5mm>
%\ar@{-}[r]^{\mc{W}}
&
*+[F-]{\text{$Z$}}
\ar@{<<.}[ul]
\\
&
*++[o][F.]{\text{\scriptsize$B_V, \theta_{V -}$}}
&
}
\notag \\[-1.95em]
&\hspace{-4.5em}
{^\text{X}
_\text{Y}}^{(-)}
\text{Z}
\label{quiverP-} \\[-.5em]
\notag
\end{align}

\paragraph{SQED$^{( \mathcal{P} - )}$ vs ${^{\text{X}}_{\text{Y}}}^{(-)}\text{Z}$}
We can define the SQED with the same parity conditions as used in SQED$^{( \mathcal{P} + )}$ but choosing the other background Wilson line phase, that is, $\theta_{J -}$. We name this case SQED$^{( \mathcal{P} - )}$ whose quiver diagram is drawn on the left side of \eqref{quiverP-}. This quiver diagram instantly gives us the index of SQED$^{( \mathcal{P} - )}$
\begin{align} %SCI for SQED
&
\mathcal{I}_{\text{SQED}^{( \mathcal{P} - )}} ( x, \alpha, B_{J} ) \notag \\ %1
&=
q^{\frac{1}{8}} \frac{( q^{2} ; q^{2} )_{\infty}}{( q ; q^{2} )_{\infty}}
\oint_{C_0} \frac{d z}{2 \pi i z} z^{s}
\left\{
a^{- \frac{1}{4}}
\frac
{( z^{- 1} a^{\frac{1}{2}} q^{\frac{1}{2}}, z a^{\frac{1}{2}} q^{\frac{1}{2}}; q^{2} )_{\infty}}
{( z a^{- \frac{1}{2}} q^{\frac{1}{2}}, z^{- 1} a^{- \frac{1}{2}} q^{\frac{1}{2}}; q^{2} )_{\infty}}
-
a^{\frac{1}{4}}
\frac
{( z^{- 1} a^{\frac{1}{2}} q^{\frac{3}{2}}, z a^{\frac{1}{2}} q^{\frac{3}{2}} ; q^{2} )_{\infty}}
{( z a^{- \frac{1}{2}} q^{\frac{3}{2}}, z^{- 1} a^{- \frac{1}{2}} q^{\frac{3}{2}} ; q^{2} )_{\infty}}
\right\}, %2
\label{scib2sqed1}
\end{align}
where all variables are defined in the same manner as $\mathcal{I}_{\text{SQED}^{( \mathcal{P} + )}}$ \eqref{scib1sqed1}. The only difference from the previous example is the relative weight originated from the BF term \eqref{BFvalue} in summing over the dynamical gauge holonomies in \eqref{CPsum}. Thus, we can proceed with the computation in a parallel way to \eqref{scib1sqed1}.

On the dual side, we call it ${^{\text{X}}_{\text{Y}}}^{(-)}\text{Z}$, although chiral fields satisfy the same parity conditions as ${^{\text{X}}_{\text{Y}}}^{(+)}\text{Z}$, they couple with the background Wilson line phase $\theta_{V -}$. %This affects the parity conditions of $X$ and $Y$ such that they are interchanged each other with an extra phase. 
The index of ${^{\text{X}}_{\text{Y}}}^{(-)}\text{Z}$ corresponding to the quiver on the right side of \eqref{quiverP-} is given by
\begin{align} %SCI for XYZ
\mathcal{I}_{{^{\text{X}}_{\text{Y}}}^{(-)}\text{Z}} ( x, \tilde{\alpha}, B_{V} )
=
q^{\frac{1}{8}} \tilde{a}^{- \frac{1}{4}}
\left( \tilde{a}^{- \frac{1}{2}} q^{\frac{1}{2}} \right)^{| \tilde{s} |}
\frac{( - \tilde{a}^{- \frac{1}{2}} q^{1 + |\tilde{s}|} ; q )_{\infty}}{( - \tilde{a}^{\frac{1}{2}} q^{|\tilde{s}|} ; q )_{\infty}}
\frac{( \tilde{a} ; q^{2} )_{\infty}}{( \tilde{a}^{- 1} q ; q^{2} )_{\infty}},
\label{scib2xyz1}
\end{align}
where we reuse the arguments $\tilde{a}$ and $\tilde{s}$ from \eqref{scib1xyz1}. The negative signs in the second fraction of \eqref{scib2xyz1} are caused by the fact that $X$, $Y$ which have U$(1)_{V}$ charges $\pm 1$ are coupled to $\theta_{V -}$.

Mirror symmetry between SQED$^{( \mathcal{P} - )}$ and ${^{\text{X}}_{\text{Y}}}^{(-)}\text{Z}$ should be realized as
\begin{align}
\mathcal{I}_{\text{SQED}^{( \mathcal{P} - )}} ( x, \alpha, B_{J} )
=
\mathcal{I}_{{^{\text{X}}_{\text{Y}}}^{(-)}\text{Z}} ( x, \tilde{\alpha}, B_{V} )
\label{mirror2}
\end{align}
under identifications $\alpha = \tilde{\alpha}^{- 1}$ and $B_{J} = B_{V}$ as before. The readers can confirm numerically two types of equivalence \eqref{mirror1} and \eqref{mirror2}. Also, they can be verified analytically by utilizing the $q$-binomial theorem \eqref{qbinomial}. We summarize mathematical tools and indicate exact proof for both examples in Appendix \ref{24mirrorsym} (see \cite{Tanaka:2014oda} for details and general arguments about the $q$-binomial theorem).



%\vspace{-2em}
%\begin{table}[b] %Parity actions in the SQED and the XYZ model
%\caption{Parity actions in SQED$^{( \mathcal{P} - )}$ and $^{\text{X}}_{\text{Y}} \text{Z}^{(-)}$ with a background $\theta_{-}$.\label{b2-type}}
%\begin{tabular}{c}
%	\hspace{2em}
%	\begin{minipage}[t]{.5\hsize} %SQED
%		\vspace{-.3em}
%		\begin{center}
%			\begin{tabular}{rcl} \hline
%			& SQED$^{( \mathcal{P} - )}$ & \\ \hline
%			$\sigma, \rho$ & $\begin{xy} {(0,5) \ar (7.5,5)} \end{xy}$ & $- \sigma, - \rho + \pi e^{2}$  \\
%			$Q$ & $\begin{xy} {(0,5) \ar (7.5,5)} \end{xy}$ & $Q$ \\
%			$\tilde{Q}$ & $\begin{xy} {(0,5) \ar (7.5,5)} \end{xy}$ & $\tilde{Q}$ \\ \hline
%			\end{tabular}
%		\end{center}
%	\end{minipage}
%	\hspace{-1.5em}
%	$\begin{xy} {(0,-10) \ar@{<=>} (10,-10)} \end{xy}$
%	\hspace{-5em}
%	\begin{minipage}[t]{.5\hsize} %XYZ
%		\vspace{-.3em}
%		\begin{center}
%			\begin{tabular}{ccc} \hline
%			& $^{\text{X}}_{\text{Y}} \text{Z}^{(-)}$ & \\ \hline
%			\shortstack{\strut $X$ \\ $Y$ } & $\begin{xy} {(0,10) \ar (7.5,5)}, {(0,5) \ar (7.5,10)} \end{xy}$ & \shortstack{\strut $- Y$ \\ $- X$ } \\
%			$Z$ & $\begin{xy} {(0,5) \ar (7.5,5)} \end{xy}$ & $Z$ \\ \hline
%			\end{tabular}
%		\end{center}
%	\end{minipage}
%\end{tabular}
%\end{table}



\clearpage
%%%%%%%%%%%% Section 3.3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{$\text{SQED}^{( \mathcal{CP} )}$ vs XYZ}\label{CPtype}
\begin{align}
%%%% SQED^CP+
\xymatrix {
&
*++[o][F.]{\text{\scriptsize$B_{A}^{+}, \theta_A$}} 
&
\\
*+[F-]{\text{\scriptsize$
\begin{matrix}
Q \\
\tilde{Q}
\end{matrix}
$}}
\ar@{.>}[ur]<1.5mm>
\ar@{.>}[ur]<-1.5mm>
&
*++[o][F-]{\text{\scriptsize$\mc{CP}$}} 
\ar@{->}[l]<1.5mm>
\ar@{<-}[l]<-1.5mm>
\ar@{.}[d]^{\text{BF}}
&
\\
&
*++[o][F.]{\text{\scriptsize$B_{J}^{+},\theta_J$}} 
&
\\
&
\text{SQED}^{(\mc{CP}+)}
&
}
\hspace{-2em}
\begin{xy}
{(5,-15) \ar @{<=>} (15,-15)}
\end{xy}
\hspace{2em}
%%%% XYZ
\xymatrix {
&
*++[o][F.]{\text{\scriptsize$\tilde{B}_{A}^{+}, \tilde{\theta}_A$}} 
\ar@{<.}[d]
\ar@{<.}[dl]
&
\\
*+[F-]{\text{$X$}} 
%\ar@{-}[r]^{\mc{W}}
\ar@{.>}[dr]
&
*+[F-]{\text{$Y$}} 
\ar@{<.}[d]
%\ar@{-}[r]^{\mc{W}}
&
*+[F-]{\text{$Z$}}
\ar@{<<.}[ul]
\\
&
*++[o][F.]{\text{\scriptsize$B_{V}^{+},\theta_V$}} 
&
}
\notag \\[-1.75em]
&\hspace{-7.5em}
\text{X}^{(+)}
\text{Y}^{(+)}
\text{Z}
\label{quiverCP+} \\[-1em]
\notag
\end{align}

\paragraph{SQED$^{( \mathcal{CP} + )}$ vs X$^{( + )}$Y$^{( + )}$Z}
Let us turn to concentrating on mirror symmetry under our new parity conditions \eqref{vecp2} and \eqref{ematp2} which act as charge conjugation $\mathcal{C}$ simultaneously with $\mathcal{P}$. Here, the background gauge field for U$(1)_{J}$ is in $\mc{P}$-type \eqref{PBG} to keep the BF term parity-even.
First, we choose it to be even-holonomy $B_{J}^{+}$ on the SQED side which we denote by SQED$^{( \mathcal{CP} + )}$. The quiver diagram of SQED$^{( \mathcal{CP} + )}$ is shown on the left side of \eqref{quiverCP+} where ($Q, \tilde{Q}$) should be treated as a doublet and provide the one-loop determinant on $\mathbb{S}^{2} \times \mathbb{S}^{1}$. Combining the contribution of the vector multiplet, the index is written\footnote{We can replace $|B_{J}|$ with $B_{J}$ in the formula \eqref{d1loop}. See the detail argument of \cite{Krattenthaler:2011da}.} as
\begin{align} %SCI for SQED
&
\mathcal{I}_{\text{SQED}^{( \mathcal{CP} + )}} ( x, \alpha, w ) \notag \\ %1
&=
\frac{1}{2} q^{- \frac{1}{8}}
\frac{( q; q^{2} )_{\infty}}{( q^{2}; q^{2} )_{\infty}}
\sum_{m \in \mathbb{Z}}
\left( a ^{\frac{1}{2}} w \right)^{m}
\left[
%\sum_{m \in \mathbb{Z}}
%\left( q^{\frac{1}{2}} a ^{- \frac{1}{2}} w \right)^{m}
\frac{( a^{\frac{1}{2}} q^{m + \frac{1}{2}}; q )_{\infty}}{( a^{- \frac{1}{2}} q^{m + \frac{1}{2}}; q )_{\infty}}
+
%\sum_{m \in \mathbb{Z}}
%\left( q^{\frac{1}{2}} a ^{- \frac{1}{2}} w \right)^{m}
\frac{( - a^{\frac{1}{2}} q^{m + \frac{1}{2}}; q )_{\infty}}{( - a^{- \frac{1}{2}} q^{m + \frac{1}{2}}; q )_{\infty}}
\right], %2
\label{scib3sqed1}
\end{align}
where we define $m = B_{J}/2$.% and $a = \alpha^{2} x^{2 \Delta}$. Note that we use $a$ with a different definition from the previous subsection. Also, $w := e^{i \theta_{J}}$ is a fugacity associated to gauged U$(1)_{J}$.

We express the dual XYZ as X$^{( + )}$Y$^{( + )}$Z because $X$ and $Y$ are coupled to the even-holonomy sector of the chosen U$(1)_{V}$ background gauge field.
Each field behaves as a single field on $\mathbb{RP}^{2} \times \mathbb{S}^{1}$ as explained in Table \ref{b3-type}. We can immediately obtain the index of X$^{( + )}$Y$^{( + )}$Z from its quiver diagram \eqref{quiverCP+} as
\begin{align} %SCI for XYZ
\mathcal{I}_{\text{X}^{( + )}\text{Y}^{( + )}\text{Z}} ( x, \tilde{\alpha}, \tilde{w} )
&=
q^{- \frac{1}{8}}
\frac
{( \tilde{a}^{- \frac{1}{2}} \tilde{w}^{- 1} q, \tilde{a}^{- \frac{1}{2}} \tilde{w} q, \tilde{a}; q^{2} )_{\infty}}
{( \tilde{a}^{\frac{1}{2}} \tilde{w}, \tilde{a}^{\frac{1}{2}} \tilde{w}^{- 1}, \tilde{a}^{- 1} q; q^{2} )_{\infty}},
\label{scib3xyz1}
\end{align}
where %$\tilde{a} := \tilde{\alpha}^{- 2} x^{2 \Delta}$ and 
$\tilde{w} := e^{i \theta_{V}}$ is a fugacity associated to U$(1)_{V}$.

$\mathcal{N} = 2$ mirror symmetry between SQED$^{( \mathcal{CP} + )}$ and X$^{( + )}$Y$^{( + )}$Z is established 
\begin{align}
\mathcal{I}_{\text{SQED}^{( \mathcal{CP} + )}} ( x, \alpha, w )
=
\mathcal{I}_{\text{X$^{(+)}$Y$^{(+)}$Z}} ( x, \tilde{\alpha}, \tilde{w} )
\label{mirror3}
\end{align}
under identifications $\alpha = \tilde{\alpha}^{- 1}$ and $w = \tilde{w}$ which are concluded from the mirror map (Table \ref{mmap}). This is a quite new relation realizing mirror symmetry on the unorientable manifold.



\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
%%%% SQED
\xymatrix {
&
*++[o][F.]{\text{\scriptsize$B_{A}^{+}, \theta_A$}} 
&
\\
*+[F-]{\text{\scriptsize$
\begin{matrix}
Q \\
\tilde{Q}
\end{matrix}
$}}
\ar@{.>}[ur]<1.5mm>
\ar@{.>}[ur]<-1.5mm>
&
*++[o][F-]{\text{\scriptsize$\mc{CP}$}} 
\ar@{->}[l]<1.5mm>
\ar@{<-}[l]<-1.5mm>
\ar@{.}[d]^{\text{BF}}
&
\\
&
*++[o][F.]{\text{\scriptsize$B_{J}^{-}, \theta_J$}}
\\
&
\text{SQED}^{(\mc{CP}-)}
&
}
\hspace{-2em}
\begin{xy}
{(5,-15) \ar @{<=>} (15,-15)}
\end{xy}
\hspace{2em}
%%%% XYZ
\xymatrix {
&
*++[o][F.]{\text{\scriptsize$\tilde{B}_{A}^{+}, \tilde{\theta}_A$}} 
\ar@{<.}[d]
\ar@{<.}[dl]
&
\\
*+[F-]{\text{$X$}} 
%\ar@{-}[r]^{\mc{W}}
\ar@{.>}[dr]
&
*+[F-]{\text{$Y$}} 
\ar@{<.}[d]
%\ar@{-}[r]^{\mc{W}}
&
*+[F-]{\text{$Z$}}
\ar@{<<.}[ul]
\\
&
*++[o][F.]{\text{\scriptsize$B_{V}^{-}, \theta_V$}}
& }
\notag \\[-1.75em]
&\hspace{-7.5em}
\text{X}^{(-)}
\text{Y}^{(-)}
\text{Z}
\label{quiverCP-} \\[-1em]
\notag
\end{align}

\paragraph{SQED$^{( \mathcal{CP} - )}$ vs X$^{( - )}$Y$^{( - )}$Z}
As the final example, we would like to mention SQED$^{( \mathcal{CP} - )}$ which is the SQED with the vector multiplet $V^{( \mathcal{CP} )}$ coupling to the fixed background gauge holonomy $B_{J}^{-}$ of U$(1)_{J}$ through the BF term. The quiver diagram of SQED$^{( \mathcal{CP} - )}$ is drawn on the lhs of \eqref{quiverCP-}. The matters $Q$ and $\tilde{Q}$ should be treated as a doublet as in SQED$^{( \mathcal{CP} + )}$, whereas a chosen $B_{J}^{-}$ produces the negative sign for the odd holonomy sector of the dynamical gauge field in summing up its configuration, which originated from the BF term \eqref{BFvalue}. This is an only difference from the previous case, therefore, we have the index of SQED$^{( \mathcal{CP} - )}$
\begin{align} %SCI for SQED
&
\mathcal{I}_{\text{SQED}^{( \mathcal{CP} - )}} ( x, \alpha, w ) \notag \\ %1
&=
\frac{1}{2} q^{- \frac{1}{8}}
\frac{( q; q^{2} )_{\infty}}{( q^{2}; q^{2} )_{\infty}}
\sum_{m \in \mathbb{Z}}
\left( a^{\frac{1}{2}} w \right)^{m}
\left[
%\sum_{m \in \mathbb{Z}}
%\left( q^{\frac{1}{2}} a^{- \frac{1}{2}} w \right)^{m}
\frac{( a^{\frac{1}{2}} q^{m + \frac{1}{2}}; q )_{\infty}}{( a^{- \frac{1}{2}} q^{m + \frac{1}{2}}; q )_{\infty}}
-
%\sum_{m \in \mathbb{Z}}
%\left( q^{\frac{1}{2}} a^{- \frac{1}{2}} w \right)^{m}
\frac{( - a^{\frac{1}{2}} q^{m + \frac{1}{2}}; q )_{\infty}}{( - a^{- \frac{1}{2}} q^{m + \frac{1}{2}}; q )_{\infty}} \right], %2
\label{scib4sqed1}
\end{align}
where we repeat to use the variables defined in $\mathcal{I}_{\text{SQED}^{( \mathcal{CP} + )}}$.

We denote the theory dual to SQED$^{( \mathcal{CP} - )}$ as X$^{( - )}$Y$^{( - )}$Z characterized by the parity conditions shown in Table \ref{b3-type} with selecting the background gauge field $B_{V}^{-}$. This coupling leads to the situation where $X$ and $Y$ belong to the odd-holonomy sector of the matter multiplet on $\mathbb{RP}^{2} \times \mathbb{S}^{1}$, while $Z$ does not receive any effect. We quote the contributions of such chiral fields from the subsection \ref{Recipe} so that the index of X$^{( - )}$Y$^{( - )}$Z is obtained as
\begin{align} %SCI for XYZ
\mathcal{I}_{\text{X}^{( - )}\text{Y}^{( - )}\text{Z}} ( x, \tilde{\alpha}, \tilde{w} )
&=
q^{\frac{3}{8}} \tilde{a}^{- \frac{1}{2}}
\frac
{( \tilde{a}^{- \frac{1}{2}} \tilde{w}^{- 1} q^{2}, \tilde{a}^{- \frac{1}{2}} \tilde{w} q^{2}, \tilde{a}; q^{2} )_{\infty}}
{( \tilde{a}^{\frac{1}{2}} \tilde{w} q, \tilde{a}^{\frac{1}{2}} \tilde{w}^{- 1} q, \tilde{a}^{- 1} q; q^{2} )_{\infty}},
\label{scib4xyz1}
\end{align}
where $\tilde{a}$ is the same one defined in the previous example.

We declare $\mathcal{N} = 2$ mirror symmetry which connects SQED$^{( \mathcal{CP} - )}$ with X$^{( - )}$Y$^{( - )}$Z on $\mathbb{RP}^{2} \times \mathbb{S}^{1}$ as the nontrivial identity
\begin{align}
\mathcal{I}_{\text{SQED}^{( \mathcal{CP} - )}} ( x, \alpha, w )
=
\mathcal{I}_{\text{X$^{(-)}$Y$^{(-)}$Z}} ( x, \tilde{\alpha}, \tilde{w} )
\label{mirror4}
\end{align}
under identifications $\alpha = \tilde{\alpha}^{- 1}$ and $w = \tilde{w}$. We provide rigorous proof of the statements \eqref{mirror3} and \eqref{mirror4} by essencially employing the Ramanujan's summation formula \eqref{rama} and the specific product-to-sum identity of the elliptic theta functions \eqref{pts4443} step by step.



%\begin{table}[b] %Charge conjugations in the SQED and the XYZ model
%\caption{Parity conditions in SQED$^{( \mathcal{CP} - )}$ accompanying charge conjugation and XYZ$^{( - )}$ with a background $\theta_{-}$.\label{b4-type}}
%\begin{tabular}{c}
%	\hspace{2em}
%	\begin{minipage}[t]{.5\hsize} %SQED
%		\vspace{-.3em}
%		\begin{center}
%			\begin{tabular}{rcl} \hline
%			& SQED$^{( \mathcal{CP} - )}$ & \\ \hline
%			$\sigma, \rho$ & $\begin{xy} {(0,5) \ar (7.5,5)} \end{xy}$ & $+ \sigma, + \rho + \pi e^{2}$  \\
%			\shortstack{\strut $Q$ \\ $\tilde{Q}$ } & $\begin{xy} {(0,10) \ar (7.5,5)}, {(0,5) \ar (7.5,10)} \end{xy}$ & \shortstack{\strut $\tilde{Q}$ \\ $Q$ } \\ \hline
%			\end{tabular}
%		\end{center}
%	\end{minipage}
%	\hspace{-2em}
%	$\begin{xy} {(0,-10) \ar@{<=>} (10,-10)} \end{xy}$
%	\hspace{-2em}
%	\begin{minipage}[t]{.35\hsize} %XYZ
%		\vspace{-.3em}
%		\begin{center}
%			\begin{tabular}{ccc} \hline
%			& XYZ$^{( - )}$ & \\ \hline
%			$X$ & $\begin{xy} {(0,5) \ar (7.5,5)} \end{xy}$ & $- X$ \\
%			$Y$ & $\begin{xy} {(0,5) \ar (7.5,5)} \end{xy}$ & $- Y$ \\
%			$Z$ & $\begin{xy} {(0,5) \ar (7.5,5)} \end{xy}$ & $Z$ \\ \hline
%			\end{tabular}
%		\end{center}
%	\end{minipage}
%\end{tabular}
%\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\include{common_supp_files/sonota/sections_end}
